ADELIE: Aligning Large Language Models on Information Extraction

Large language models (LLMs) usually fall short on information extraction (IE) tasks and struggle to follow the complex instructions of IE tasks. This primarily arises from LLMs not being aligned with humans, as mainstream alignment datasets typically do not include IE data. In this paper, we introduce ADELIE (Aligning large language moDELs on Information Extraction), an aligned LLM that effectively solves various IE tasks, including closed IE, open IE, and on-demand IE. We first collect and construct a high-quality alignment corpus IEInstruct for IE. Then we train ADELIE_SFT using instruction tuning on IEInstruct. We further train ADELIE_SFT with direct preference optimization (DPO) objective, resulting in ADELIE_DPO. Extensive experiments on various held-out IE datasets demonstrate that our models (ADELIE_SFT and ADELIE_DPO) achieve state-of-the-art (SoTA) performance among open-source models. We further explore the general capabilities of ADELIE, and experimental results reveal that their general capabilities do not exhibit a noticeable decline. We will release the code, data, and models to facilitate further research.

==> Fig/analysis_IE_rate.tex <==



==> Table/analysis_ablation.tex <==
\begin{table}[]
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc|c}
\toprule
                         & Closed IE & Open IE & On-demand IE& AVG \\ \midrule
\ourmodel &     $42.6$    &  $46.7$   &    $60.4$      &  $47.5$ \\
\midrule
w/o FewShot        &    $34.4$  &   $29.8$    &  $60.9$   &   $39.2$      \\
% w/o Explanation    &    $42.3$  &   $47.1$    &  $61.6$   &   $47.7$      \\
w/o Schema Aug          &  $40.7$     &  $44.7$  &   $61.2$    & $46.2$    \\
w/o Format Aug          &   $42.1$    &  $44.8$  &    $60.5$  &  $46.8$  \\
\bottomrule
\end{tabular}
}
\caption{\label{tab:ablation}Ablation Study.}
\end{table}

==> Table/training_datasets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]
% \centering
% \small{
% \scalebox{0.9}{
% \begin{tabular}{l|llll}
% \toprule
% Task                 & Datasets               & N$_{\text{Schema}}$               & N$_{\text{Inst}}$                & N$_{\text{Exp}}$             \\ \midrule
% \multirow{4}{*}{NER} & CoNLL-2003             & 4                     & 5,000                                         \\
%                      & ACE2005$_{\text{NER}}$ & 45                    & 5,000                                         \\
%                      & Ontonotes 5            & 18                    & 5,000                                         \\
%                      &                        &                       & 5,000                                         \\ \midrule
% \multirow{2}{*}{RC}  & TACRED                 & 42                    & 5,000                                         \\
%                      & FewRel                 & 20                    & 5,000                                         \\ \midrule
% RE                   &                        &                       & 5,000                                         \\ \midrule
% \multirow{2}{*}{ED}  & ACE2005$_{\text{ED}}$  & 33                    & 4,067                                          \\
%                      & MAVEN~\cite{wang2020maven}                  & 167                   & 5,000                                         \\ \midrule
% \multirow{3}{*}{EAE} & ACE2005$_{\text{EAE}}$ & 35                    & 4,420                                          \\
%                      & RAMS                   & 65                    & 5,000                                          \\
%                      & Maven-arg~\cite{wang2023maven}              & 143                   & 5,000                                         \\ \midrule
% EE                   &                        &                       & 5,000  \\ \midrule
% ERE                  & MAVEN-ERE~\cite{wang2022maven}              & 10                    & 4,278                                         \\ \midrule
% ODIE           & INSTRUCTIE~\cite{Jiao2023InstructAE}             & \multicolumn{1}{r}{-} & 4,904                                         \\ \midrule
% OpenIE               & OpenIE4                & \multicolumn{1}{r}{-} & 5,000                                        
% \\ \bottomrule
% \end{tabular}
% }
% }
% \caption{Detailed information for the \ourdata dataset. The table displays the number of schemas for each dataset (N$_{\text{Schema}}$), the number of instances collected (N$_{\text{Inst}}$), and the number of high-quality explanations generated using GPT-4 (N$_{\text{Exp}}$).{\color{red} [citation and some datasets empty.]}}
% \label{table:datasets}
% \end{table}


\begin{table*}[]
\centering
\small{
\begin{tabular}{c|lrr}
\toprule
Task                & Datasets               & N$_{\text{Schema}}$             & N$_{\text{Inst}}$                       \\ \midrule
\multirow{4}{*}{NER} & CoNLL-2003~\cite{sang2003introduction}             & 4                     & 5,000                                         \\
                     & ACE2005$_{\text{NER}}$~\cite{ace2005} & 45                    & 5,000                                         \\
                     & Ontonotes 5~\cite{pradhan2013towards}            & 18                    & 5,000                                         \\
                     &                        &                       & 5,000                                         \\ \midrule
\multirow{2}{*}{RC}  & TACRED~\cite{zhang2017position}                 & 42                    & 5,000                                         \\
                     & FewRel~\cite{han2018fewrel}                 & 20                    & 5,000                                         \\ \midrule
RE                   &                        &                       & 5,000                                         \\ \midrule
\multirow{2}{*}{ED}  & ACE2005$_{\text{ED}}$~\cite{ace2005}  & 33                    & 4,067                                          \\
                     & MAVEN~\cite{wang2020maven}                  & 167                   & 5,000                                         \\ \midrule
\multirow{3}{*}{EAE} & ACE2005$_{\text{EAE}}$~\cite{ace2005} & 35                    & 4,420                                          \\
                     & RAMS~\cite{li2021document}                   & 65                    & 5,000                                          \\
                     & Maven-arg~\cite{wang2023maven}              & 143                   & 5,000                                         \\ \midrule
EE                   &                        &                       & 5,000  \\ \midrule
ERE                  & MAVEN-ERE~\cite{wang2022maven}              & 10                    & 4,278                                         \\ \midrule
ODIE           & INSTRUCTIE~\cite{Jiao2023InstructAE}             & \multicolumn{1}{r}{-} & 4,904                                         \\ \midrule
OpenIE               & OpenIE6~\cite{kolluru2020openie6}                & \multicolumn{1}{r}{-} & 5,000                                        
\\ \bottomrule
\end{tabular}
}
\caption{Detailed information for the \ourdata dataset. The table displays the number of schemas other than "None of the above" (N$_{\text{Schema}}$) and the number of instances collected (N$_{\text{Inst}}$) for each dataset.{\color{red} [citation and some datasets empty.]}}
% \label{table:datasets}
\end{table*}

==> latex/background.tex <==
\section{Background}
This section briefly introduces all the IE tasks involved in this paper.









% 除了Cloced IE和open IE，A提出了On-demand IE，目标是从无结构化文本中抽取出用户desired的信息，比如抽取出水果的shape and taste，并整理成结构化的表格形式。On-demand IE的形式更加 flexible，更贴近现实中的需求。在本篇论文中，我们考虑了所有的IE任务，希望能够通过对齐增强模型解决这些任务的能力。







% 传统的IE任务主要分为2类：closed IE和open IE。Closed IE要求从非结构化文本周抽取出结构化的信息，通常要求抽取的信息符合a predefined schema，包含set of categories。
% 而open IE任务也是非结构化文本中抽取出n-arg relation tuples，但是依赖predefined schema。

% 除了这两类IE任务，A还提出了on-demand IE任务，

% Closed IE refers to tasks that involve a predefined set of categories, i.e., schema, where models need to give predictions based on these categories。而open IE任务通常







